Autonomous tuning and charge state detection of gate defined quantum dots

Defining quantum dots in semiconductor based heterostructures is an essential step in initializing solid-state qubits. With growing device complexity and increasing number of functional devices required for measurements, a manual approach to finding suitable gate voltages to confine electrons electrostatically is impractical. Here, we implement a two-stage device characterization and dot-tuning process which first determines whether devices are functional and then attempts to tune the functional devices to the single or double quantum dot regime. We show that automating well established manual tuning procedures and replacing the experimenter's decisions by supervised machine learning is sufficient to tune double quantum dots in multiple devices without pre-measured input or manual intervention. The quality of measurement results and charge states are assessed by four binary classifiers trained with experimental data, reflecting real device behaviour. We compare and optimize eight models and different data preprocessing techniques for each of the classifiers to achieve reliable autonomous tuning, an essential step towards scalable quantum systems in quantum dot based qubit architectures.

==> tables/hyperparameters_DecisionTreeClassifier.tex <==
\begin{tabular}{lcccc}
\toprule
   hyper parameter & pinchoff & singledot & doubledot & dotregime \\
\hline
         criterion &     gini &   entropy &   entropy &   entropy \\
      max features &     auto &      None &      sqrt &      auto \\
  min samples leaf &        2 &         3 &         3 &         1 \\
 min samples split &        6 &         2 &         6 &         2 \\
          splitter &   random &      best &      best &    random \\
\bottomrule
\end{tabular}


==> tables/hyperparameters_KNeighborsClassifier.tex <==
\begin{tabular}{lcccc}
\toprule
hyper parameter &  pinchoff & singledot & doubledot & dotregime \\
\hline
      algorithm &      auto &      auto &      auto &      auto \\
      leaf size &        10 &        10 &        10 &        10 \\
    n neighbors &         2 &         2 &         2 &         2 \\
              p &         3 &         2 &         1 &         2 \\
        weights &  distance &  distance &  distance &   uniform \\
\bottomrule
\end{tabular}


==> tables/hyperparameters_LogisticRegression.tex <==
\begin{tabular}{lcccc}
\toprule
hyper parameter &   pinchoff &  singledot &  doubledot &  dotregime \\
\hline
              C &        100 &        0.1 &         10 &          1 \\
   class weight &       None &       None &   balanced &   balanced \\
  fit intercept &       True &       True &       True &       True \\
       max iter &       1000 &       1000 &       1000 &       1000 \\
        penalty &         l1 &         l1 &         l2 &         l2 \\
         solver &  liblinear &  liblinear &  newton-cg &  liblinear \\
\bottomrule
\end{tabular}


==> tables/hyperparameters_MLPClassifier.tex <==
\begin{tabular}{lcccc}
\toprule
    hyper parameter &  pinchoff & singledot & doubledot & dotregime \\
\hline
         activation &      relu &      relu &      None &      None \\
              alpha &    0.0001 &       0.1 &      None &      None \\
         batch size &       100 &       300 &      None &      None \\
 hidden layer sizes &     [100] &     [100] &      None &      None \\
      learning rate &  constant &  adaptive &      None &      None \\
           max iter &      3000 &      3000 &      None &      None \\
            power t &       0.1 &       0.6 &      None &      None \\
             solver &     lbfgs &       sgd &      None &      None \\
\bottomrule
\end{tabular}


==> tables/hyperparameters_RandomForestClassifier.tex <==
\begin{tabular}{lcccc}
\toprule
   hyper parameter & pinchoff & singledot & doubledot & dotregime \\
\hline
         criterion &     gini &      None &   entropy &      gini \\
      max features &     auto &      None &      auto &      log2 \\
  min samples leaf &        1 &      None &         1 &         2 \\
 min samples split &        6 &      None &         2 &         2 \\
      n estimators &       10 &      None &       100 &       100 \\
\bottomrule
\end{tabular}


==> tables/hyperparameters_SVC.tex <==
\begin{tabular}{lcccc}
\toprule
hyper parameter & pinchoff & singledot & doubledot & dotregime \\
\hline
              C &     1000 &       0.1 &       0.1 &       0.1 \\
          gamma &        1 &       0.1 &       0.1 &       0.1 \\
         kernel &      rbf &      poly &      poly &    linear \\
\bottomrule
\end{tabular}

